CamPilot: A Multi-Agent Cinematic Assistant for Camera-Controlled Movie Generation

The integration of large language models (LLMs) into video generation has enabled rapid text-to-video creation and improved visual quality. However, it still falls short of professional filmmaking, where cinematographic language is less refined than human-crafted camera work and multi-shot continuity remains challenging. To address these limitations, we introduce CamPilot, a multi-agent framework that integrates cinematographic planning and camera-work control to produce more coherent, logically structured, and human-aesthetic movies. CamPilot adopts a GRPO-based learning paradigm to learn camera work planning from 14K real-world professional movies, internalizing motion patterns and composition principles that support reasoning over shooting techniques (e.g., camera angle, motion, and focal behavior) and cross-shot relationships for controllable camera-viewpoint generation. Multiple agents further collaborate and evolve to improve overall output quality. To support this work and further studies in this domain, we establish CamEval, a benchmark for evaluating camera work quality and cinematic engagement. Empirical results show that CamPilot outperforms state-of-the-art text-to-movie generation methods on cinematographic control and quality, highlighting the impact of professional camera design on movie generation.

==> header.tex <==

\newcommand{\draftonly}[1]{#1}
\newcommand{\draftcomment}[3]{\draftonly{\textcolor{#2}{{{[#1: #3]}}}}}
\newcommand{\mz}[1]{\draftcomment{Mengzhou}{purple}{#1}}
\newcommand{\sm}[1]{\draftcomment{Sadhika}{blue}{#1}}
\newcommand{\danqi}[1]{\draftcomment{Danqi}{orange}{#1}}
\newcommand{\suchin}[1]{\draftcomment{Suchin}{red}{#1}}

\newcommand{\cmark}{\checkmark}%
\newcommand{\xmark}{ }%
\newcommand{\flan}{\textsc{Flan V2}}
\newcommand{\cott}{\textsc{CoT}}
\newcommand{\dolly}{\textsc{Dolly}}
\newcommand{\hh}{\textsc{HH}}
\newcommand{\humaneval}{\textsc{HumanEval}}
\newcommand{\oasst}{\textsc{Open Assistant 1}}
\newcommand{\gsm}{\textsc{GSM}}
\newcommand{\shp}{\textsc{SHP}}
\newcommand{\se}{\textsc{SE}}
\newcommand{\gptalpaca}{\textsc{GPT4-Alpaca}}
\newcommand{\llamasmall}{\textsc{Llama-2-7B}}
\newcommand{\llamalarge}{\textsc{Llama-2-13B}}


\newcommand{\llamab}{\textsc{Llama-2-7B}}
\newcommand{\llamac}{\textsc{Llama-2-13B}}
\newcommand{\llamad}{\textsc{Llama-3-8B}}
\newcommand{\llamadinst}{\textsc{Llama-3-8B-Instruct}}
\newcommand{\llamae}{\textsc{Llama-3.1-8B}}
\newcommand{\llamaeinst}{\textsc{Llama-3.1-8B-Ins.}}
\newcommand{\mistralav}{\textsc{Mistral-7B-v0.1}}
\newcommand{\mistralavinst}{\textsc{Mistral-7B-Instruct-v0.1}}
\newcommand{\mistralb}{\textsc{Mistral-7B-v0.3}}
\newcommand{\mistralbinst}{\textsc{Mistral-7B-Ins.-v0.3}}





\newcommand{\mistral}{\textsc{Mistral-7B}}
\newcommand{\llamasmallchat}{\textsc{Llama-2-7B-Chat}}

\newcommand{\random}{Random}
\newcommand{\simdiv}{Sim + Div}
\newcommand{\simi}{Sim}
\newcommand{\less}{LESS}
\newcommand{\ours}{PU-ADKA}

\newcommand{\piref}{\pi_\text{ref}}


\definecolor{c1}{cmyk}{0,0.6175,0.8848,0.1490}
\definecolor{c2}{cmyk}{0.1127,0.6690,0,0.4431}
\definecolor{c3}{cmyk}{0.3081,0,0.7209,0.3255}
\definecolor{c4}{cmyk}{0.6765,0.2017,0,0.0667}
\definecolor{c5}{cmyk}{0,0.8765,0.7099,0.3647}

% Define colour boxes.
% Taken from https://arxiv.org/abs/2103.00453.
% \newtcbox{\hlprimarytab}{on line, rounded corners, box align=base, colback=c3!10,colframe=white,size=fbox,arc=3pt, before upper=\strut, top=-2pt, bottom=-4pt, left=-2pt, right=-2pt, boxrule=0pt}
% \newtcbox{\hlsecondarytab}{on line, box align=base, colback=red!10,colframe=white,size=fbox,arc=3pt, before upper=\strut, top=-2pt, bottom=-4pt, left=-2pt, right=-2pt, boxrule=0pt}

% \newtcbox{\flatbox}{on line, box align=base, colback=c4!10,colframe=white,size=fbox,arc=3pt, before upper=\strut, top=-2pt, bottom=-4pt, left=-2pt, right=-2pt, boxrule=0pt}

% Define up and down arrow commands.
\newcommand{\dashifted}{\raisebox{0.5\depth}{\tiny$\downarrow$}}
\newcommand{\uashifted}{\raisebox{0.5\depth}{\tiny$\uparrow$}}
\newcommand{\best}[1]{\textbf{\textcolor[RGB]{205,83,76}{#1}}}
\newcommand{\secondb}[1]{\textbf{\textcolor[RGB]{0,115,194}{#1}}}
% switched
\newcommand{\ua}[1]{{\small\hlprimarytab{\uashifted{#1}}}}
\newcommand{\da}[1]{{\small\hlsecondarytab{\dashifted{#1}}}}
\newcommand{\fa}[1]{{\small\flatbox{{#1}}}}
% switched

\newcommand{\uag}[1]{{\scriptsize\hlprimarytab{\uashifted{#1}}}}
\newcommand{\dab}[1]{{\scriptsize\hlsecondarytab{\dashifted{#1}}}}

\newcommand*{\TakeFourierOrnament}[1]{{%
\fontencoding{U}\fontfamily{futs}\selectfont\char#1}}
\newcommand*{\danger}{\TakeFourierOrnament{66}}

% \newcommand{\smallmodel}{\textsc{125m}}
% \newcommand{\medmodel}{\textsc{1.3b}}
% \newcommand{\largemodel}{\textsc{6.7b}}
% \newcommand{\xlmodel}{\textsc{13b}}
% \newcommand{\xxlmodel}{\textsc{30b}}
% \newcommand{\xxxlmodel}{\textsc{175b}}
% \newcommand{\ppl}{\textsc{ppl}}

\definecolor{gg}{HTML}{0F9D58}
\definecolor{rr}{HTML}{DB4437}
\definecolor{bb}{HTML}{4285F4}

% \newcommand{\flanv2}{\textsc{FLAN}}

\def\dsub{{\gD_{\text{train}}}}
\def\dfull{{\gD}}
\def\dval{{\gD_{\text{val}}}}
\def\dwarmup{{\gD_{\text{warmup}}}}
\newcommand{\valsub}[1]{{\gD_{\text{val}}^{(#1)}}}
\newcommand{\dtest}{\gD_{\text{test}}}
\def\numval{{m}}
\def\dim{{d}}
\newcommand{\grad}[2]{\nabla\ell(#1;#2)}
\newcommand{\loragrad}[2]{\hat\nabla\ell(#1;#2)}
\newcommand{\avggrad}[1]{\bar\nabla\ell(#1)}
\newcommand{\projgrad}[2]{\tilde\nabla\ell(#1;#2)}
\newcommand{\match}[2]{\gM(#1,#2)}
\newcommand{\diverse}[2]{\gK(#1,#2)}
\newcommand{\update}[2]{\Gamma(#1, #2)}
\newcommand{\loraupdate}[2]{\hat\Gamma(#1, #2)}
\newcommand{\approxupdate}[2]{\tilde\Gamma(#1, #2)}
\newcommand{\infadam}{{\textrm{Inf}_{\text{Adam}}}}
\newcommand{\infsgd}{{\textrm{Inf}_{\text{SGD}}}}

\newcommand{\std}[1]{\text{\scriptsize{(#1)}}}



==> tables/ablation_study_module.tex <==
\begin{table*}[t]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{@{}llcccccccc@{}}
        \toprule
        \multirow{2}{*}[-1ex]{LLM Backbone} 
        & \multirow{2}{*}[-1ex]{Method} 
        & \multicolumn{4}{c}{Camera Work Classification (\%)~$\uparrow$} 
        & \multicolumn{2}{c}{Keyframe Generation (\%)~$\uparrow$} & \multicolumn{2}{c}{Movie Generation (\%)~$\uparrow$} \\
        \cmidrule(lr){3-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
        & & Macro-Acc & Macro-Rec & Macro-Prec & Macro-F1 
          & CLIP & Inception & Consistency & Smoothness \\
        \midrule

        \multirow{5}{*}{Llama-3.1-8B-Instruct} 
            & CamPilot w/o Character Bank     &  &  &  &  &  &  &  &  \\
            & CamPilot w/o GRPO         &  &  &  &  &  &  &  &  \\
            & CamPilot w/o Reviser              &  &  &  &  &  &  &  &  \\
            & \textbf{CamPilot (Ours)} &  &  &  &  &  &  &  &  \\
        \bottomrule
    \end{tabular}
    }
    \caption{Ablation study results with Automatic metrics on camera work classification and keyframe/movie generation. The mean (std) over three random runs is reported. The best results are shown in \textbf{bold}, and the second-best are \underline{underlined}.}
    \label{tab:ablation_study_module}
\end{table*}










==> tables/usability_testing.tex <==
\begin{table}[ht]
  \centering
  \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lccc}
      \toprule
      Method & Cinematography & Consistency & Aesthetics \\
      \midrule
      MovieAgent &  &  &  \\
      CamPilot   &  &  &  \\
      \bottomrule
    \end{tabular}
  }
  \caption{Results of usability testing.}
  \label{tab:usability}
\end{table}

